A Survey on Resilience in the IoT: Taxonomy, Classification and Discussion of Resilience Mechanisms

Internet-of-Things (IoT) ecosystems tend to grow both in scale and complexity as they consist of a variety of heterogeneous devices, which span over multiple architectural IoT layers (e.g., cloud, edge, sensors). Further, IoT systems increasingly demand the resilient operability of services as they become part of critical infrastructures. This leads to a broad variety of research works that aim to increase the resilience of these systems. In this paper, we create a systematization of knowledge about existing scientific efforts of making IoT systems resilient. In particular, we first discuss the taxonomy and classification of resilience and resilience mechanisms and subsequently survey state-of-the-art resilience mechanisms that have been proposed by research work and are applicable to IoT. As part of the survey, we also discuss questions that focus on the practical aspects of resilience, e.g., which constraints resilience mechanisms impose on developers when designing resilient systems by incorporating a specific mechanism into IoT systems.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> diagrams/mechanismlayer.tex <==
\begin{tikzpicture}
\footnotesize 
		% Vertical distance 
		\newcommand{\vdist}{0.7}
		
		% Horizontal distance
		\newcommand{\hdist}{1.7}
		
		% Length of bars
		\newcommand{\barb}{1}
		\newcommand{\bare}{9}
		
		% Placement of text 
		\newcommand{\textb}{11}

		\tikzset{dot/.style={fill=black,circle}}

		% Device
		\node[] at (\textb,3.7){\textbf{Sensor Landscape}};
		\draw[dashed] (\barb,3.7) -- (\bare,3.7);
		
		\foreach\l[count=\y] in {Lightweight Encryption,Plausability Checks, Device Redundancy}
		{
			\draw (\barb,\y*\vdist+1) -- (\bare,\y*\vdist+1);
			\node at (\textb,\y*\vdist+1){\l};
		}
		
		\foreach\l[count=\x] in {Confidentiality,Integrity,Reliability,Safety,Maintainability}
		{
			\draw (\x*\hdist,0) -- (\x*\hdist,3.7);
			\node at (\x*\hdist,4){\l};
		}
	
	
		\node[dot] at (3*\hdist,3*\vdist+1){};
		\node[dot] at (2*\hdist,3*\vdist+1){};
		\node[dot] at (4*\hdist,3*\vdist+1){};
		\node[dot] at (2*\hdist,2*\vdist+1){};
		\node[dot] at (4*\hdist,2*\vdist+1){};
		\node[dot] at (1*\hdist,1*\vdist+1){};
		
		% Edge
		\node[] at (\textb,1){\textbf{Edge}};
		\draw[dashed] (\barb,1) -- (\bare,1);
		
		\foreach\l[count=\y] in {Active Replication, Intrusion Detection Systems, Monitoring}
		{
			\draw (\barb,\y*\vdist-1.7) -- (\bare,\y*\vdist-1.7);
			\node at (\textb,\y*\vdist-1.7){\l};
		}
		
		\foreach\l[count=\x] in {Confidentiality,Integrity,Reliability,Safety,Maintainability}
		{
			\draw (\x*\hdist,-3) -- (\x*\hdist,0);
		%	\node at (\x*2.2,4.5){\l};
		}
		
		
			\node[dot] at (5*\hdist,3*\vdist-1.7){};
			\node[dot] at (3*\hdist,3*\vdist-1.7){};
		
		\node[dot] at (2*\hdist,2*\vdist-1.7){};
		\node[dot] at (5*\hdist,2*\vdist-1.7){};
		\node[dot] at (2*\hdist,1*\vdist-1.7){};
		\node[dot] at (3*\hdist,1*\vdist-1.7){};
		
		% Core
		\node[] at (\textb,-1.7){\textbf{Core}};
		\draw[dashed] (\barb,-1.7) -- (\bare,-1.7);
		
		\foreach\l[count=\y] in {Virtual Machine Introspection, Snapshots, Transport Layer Security}
		{
			\draw (\barb,\y*\vdist-4.5) -- (\bare,\y*\vdist-4.5);
			\node at (\textb,\y*\vdist-4.5){\l};
		}
		
		\foreach\l[count=\x] in {Confidentiality,Integrity,Reliability,Safety,Maintainability}
		{
			\draw (\x*\hdist,-4) -- (\x*\hdist,0);
			%	\node at (\x*2.2,4.5){\l};
		}
		
		\node[dot] at (1*\hdist,3*\vdist-4.5){};
		\node[dot] at (2*\hdist,3*\vdist-4.5){};
		
		\node[dot] at (5*\hdist,2*\vdist-4.5){};
		\node[dot] at (2*\hdist,2*\vdist-4.5){};
		
		\node[dot] at (3*\hdist,1*\vdist-4.5){};
		\node[dot] at (2*\hdist,1*\vdist-4.5){};
		
	\end{tikzpicture}
